RaySplats: Ray Tracing based Gaussian Splatting

3D Gaussian Splatting (3DGS) is a process that enables the direct creation of 3D objects from 2D images. This representation offers numerous advantages, including rapid training and rendering. However, a significant limitation of 3DGS is the challenge of incorporating light and shadow reflections, primarily due to the utilization of rasterization rather than ray tracing for rendering. This paper introduces RaySplats, a model that employs ray-tracing based Gaussian Splatting. Rather than utilizing the projection of Gaussians, our method employs a ray-tracing mechanism, operating directly on Gaussian primitives represented by confidence ellipses with RGB colors. In practice, we compute the intersection between ellipses and rays to construct ray-tracing algorithms, facilitating the incorporation of meshes with Gaussian Splatting models and the addition of lights, shadows, and other related effects.

==> flametabelka.tex <==
\begin{table}[H]
{\small 
\begin{center}
    \begin{tabular}{lllllll}
    \multicolumn{7}{c}{ PSNR $\uparrow$}
 \\ \hline
    %\addtolength{\tabcolsep}{-0.4cm}
     Person &\hspace*{-0.2cm} 1&\hspace*{-0.2cm} 2&  \hspace*{-0.2cm} 3&\hspace*{-0.2cm} 4&\hspace*{-0.2cm}5&\hspace*{-0.2cm} 6 
 \\ \hline

\multicolumn{7}{c}{Static}
 \\ \hline
 
\arrayrulecolor{lightgray}\hline \arrayrulecolor{black}
 NeRF  & 33.37 & 33.39 &33.08 &31.96 & 33.15 &32.42  \\
 GS &50.16&49.04&49.81&49.97&49.77&49.17\\\hline

\multicolumn{7}{c}{Editable}
 \\ 
  NeRFlame  & 27.89 & 29.79  & 29.70 & 25.78  &32.59 & 29.18   \\
%&\our{}\scalebox{.8}{$_{100}$} - B  & 38.62 &  39.27 &  39.56 & 36.83 &  40.60 &  38.96  \\
%\our{}&  \bf 31.65 & \bf  29.54  &  \bf 30.66 &   \bf 29.91 &  \bf 32.32 &  \bf 29.98  \\ 
\our{}&  \bf 32.73 & 29.56 & 29.42 & \bf 29.95 & 32.27  & \bf 31.50 \\ 
%&\our{}\scalebox{.8}{$_{300}$} - W  & 32.88 & 31.06  &   & 31.40  & 33.18 & 28.7   
% \our{}&  \bf 31.65 & \bf  29.54  &  \bf 30.66 &   \bf 29.91 &  \bf 32.32 &  \bf 29.98  \\ 
% \multicolumn{8}{l}{}\\
%  \hline
% \multicolumn{8}{l}{ SSIM $\uparrow$ }
%  \\ \hline
% \multirow{3}{*}{A}  &NeRFlame  & 0.95 & 0.96  & 0.96 &0.92  & 0.96 &0.95   \\
% %&\our{}\scalebox{.8}{$_{100}$}$^B$  & 0.98 & 0.98 & 0.97 &0.97& 0.98 & 0.98  \\
% &\our{} & 0.97 & 0.96 &  0.97 &0.96 &0.98  &0.96   \\
% %&\our{}\scalebox{.8}{$_{300}$}$^W$ & 0.98 &  0.97 &   & 0.97& &    \\
% \arrayrulecolor{lightgray}\hline \arrayrulecolor{black}
% \multirow{2}{*}{S}  &NeRF  & 0.96  &0.96  & 0.97  &0.96  &0.96  &0.96    \\
% &GS &0.99 &0.99&0.99&0.99&0.99& 0.99
% \multicolumn{8}{l}{}\\
%  \hline
% \multicolumn{8}{l}{ LPIPS $\downarrow$ }
%  \\ \hline
% \multirow{3}{*}{A}  &NeRFlame  & 0.09 & 0.06 & 0.08 &0.10 & 0.05  & 0.07  \\
% %&\our{}\scalebox{.8}{$_{100}$}$^B$ & 0.04 &  0.03 &  0.04 &  0.05& 0.03 & 0.04   \\
% &\our{}& 0.04 & 0.04 &0.04 & 0.05 & 0.03 & 0.04  \\ 
% %&\our{}\scalebox{.8}{$_{300}$}$^W$& & 0.03 & 0.03  &   & & 0.05 &    \\\\
% \arrayrulecolor{lightgray}\hline \arrayrulecolor{black}
% \multirow{2}{*}{S}  & NeRF  & 0.05  & 0.05 &0.04 &0.04 &0.05  &0.06   \\
% &GS &0.003&0.002&0.006&0.003&0.006&0.003 
    \end{tabular}
    \end{center}
    }
    % \vspace{-0.3cm}
    \caption{ Comparison of PSNR, SSIM, and LPIPS matrices between static models: NeRF, GS and referring to them: NeRFlame and \our{}. We used 100 Gaussians per face.}
    \label{tab:facescomparisionnerflame}
\end{table} 
